Visually Grounded Speech Models for Low-resource Languages and Cognitive Modelling

This dissertation examines visually grounded speech (VGS) models that learn from unlabelled speech paired with images. It focuses on applications for low-resource languages and understanding human language acquisition. We introduce a task called visually prompted keyword localisation to detect and localise keywords in speech using images. We demonstrate the effectiveness of VGS models in few-shot learning scenarios for low-resource languages like Yoruba. Additionally, we examine the mutual exclusivity bias in VGS models. Our monolingual VGS model exhibits this bias, but we found that multilingualism does not affect the bias in this VGS model similarly to what is observed in children.

==> appendices/appendices.tex <==
\input{appendices/an_appendix}

==> background/a_section.tex <==
\graphicspath{{figures/}}

\mysection{Unimodal few-shot learning}{Unimodal Few-Shot Learning}
\label{sec:unimodal_few-shot_learning}

Some text. 
\mydefinition{An apple}{is a type of fruit.} 
Some more text.
Then a figure which will be placed either at the top or bottom of a page.

\begin{figure*}[tb]
	
	\begin{minipage}[htb!]{1.0\textwidth}
		\centering
		\includegraphics[width=\textwidth]{buckeye_cropped.pdf}
		%		\vspace*{-6pt}
	\end{minipage}
	\caption{Isolating the words in the conversational spoken sequences of the Buckeye corpus.}
	\label{fig:buckeye}
	
	%	\vspace*{-5pt}
\end{figure*}

\subsection[Siamese neural networks]{Siamese Neural Networks}
\label{sec:siamese}

Check the tex file on how to define a nomenclature item like $\boldsymbol{\mathrm{z}}^{(i)}$ \nomenclature[v]{$\boldsymbol{\mathrm{z}}^{(i)}$}{A feature representation.} or $\boldsymbol{\mathrm{x}}_{\textrm{pair}}$\nomenclature[v]{$\boldsymbol{\mathrm{x}}_{\textrm{pair}}$}{A pair of $\boldsymbol{\mathrm{x}}$.}.
You can define the nomenclature variables when you first define it. Use ``v'' for variables, ``f'' for functions and ``c'' for constants.

Then you can do some math like a triplet loss: 
\begin{equation}
\begin{split}
l_{\textrm{triplet}}(\boldsymbol{\mathrm{x}}, \boldsymbol{\mathrm{x}}_{\textrm{pair}}, \boldsymbol{\mathrm{x}}_{\textrm{neg}}) & = \mathrm{max}\{0, m+d(\boldsymbol{\mathrm{x}}, \boldsymbol{\mathrm{x}}_{\textrm{pair}})-d(\boldsymbol{\mathrm{x}}, \boldsymbol{\mathrm{x}}_{\textrm{neg}})\},
\end{split}	
\end{equation} 
where 
\begin{equation}
\begin{split}
d(\boldsymbol{\mathrm{x}}_{1}, \boldsymbol{\mathrm{x}}_{2}) & = \begin{Vmatrix}\boldsymbol{\mathrm{z}}_{1} - \boldsymbol{\mathrm{z}}_{2}\end{Vmatrix}_2^2 \\
& = \begin{Vmatrix}f_{\boldsymbol{\Theta}}(\boldsymbol{\mathrm{x}}_{1}) - f_{\boldsymbol{\Theta}}(\boldsymbol{\mathrm{x}}_{2})\end{Vmatrix}_2^2
\end{split}	
\end{equation} is the squared Euclidean distance between the embeddings $\mathbf{z}_1$ and $\mathbf{z}_2$ corresponding to $\mathbf{x}_1$ and $\mathbf{x}_2$ and $m$ is some margin parameter~\cite{wang_learning_2014,hermann_multilingual_2014}.

\section{Using the acro package}
\label{sec:acro}

Define the acronyms in the \verb+fronmatter/define_acronyms.tex+ file. 

\begin{table}[!h]
	\renewcommand{\arraystretch}{1.1}
	\centering
	\caption{This table shows the different possible commands to use with acronyms.}
	\begin{tabularx}{\linewidth}{@{}llll@{}}
		\toprule
		& \multicolumn{3}{C}{Output of acro commands for acronyms when the acronyms are used for the first time. The actual acronym form is given by the ``long'' form specified in \verb+\DeclareAcronym+.} \\
		\cmidrule(lr){2-4}
		Command    & \acl{CAE} & \acl{MTriplet}\\
		\midrule 
		\acresetall
		\verb+\ac+ & \ac{CAE} & \ac{MTriplet}\\
		\acresetall
		\verb+\Ac+ & \Ac{CAE} & \Ac{MTriplet}\\
		\acresetall
		\verb+\acl+ & \acl{CAE} & \acl{MTriplet}\\
		\acresetall
		\verb+\Acl+ & \Acl{CAE} & \Acl{MTriplet}\\
		\acresetall
		\verb+\acf+ & \acf{CAE} & \acf{MTriplet}\\
		\acresetall
		\verb+\Acf+ & \Acf{CAE} & \Acf{MTriplet}\\
		\acresetall
		\verb+\acp+   & \acp{CAE} & \acp{MTriplet}\\
		\acresetall
		\verb+\Acp+ & \Acp{CAE} & \Acp{MTriplet}\\
		\acresetall
		\verb+\acfp+ & \acfp{CAE} & \acfp{MTriplet}\\
		\acresetall
		\verb+\Acfp+ & \Acfp{CAE} & \Acfp{MTriplet}\\
		\acresetall
		\verb+\aca+ & \aca{CAE} & \aca{MTriplet}\\
		\bottomrule
	\end{tabularx}
	\label{tbl:acro_first_time_examples}
\end{table}
\newpage
\begin{table}[!h]
	\renewcommand{\arraystretch}{1.1}
	\centering
	\caption{This table shows the different possible commands to use with acronyms.}
	\begin{tabularx}{\linewidth}{@{}llll@{}}
		\toprule
		& \multicolumn{3}{C}{The output of acro commands for each subsequent use (after the first use).} \\
		\cmidrule(lr){2-4}
		Commands    & \acl{AE} & \acl{MTriplet}\\
		\midrule 
		\verb+\ac+ & \ac{CAE} & \ac{MTriplet}\\
		\verb+\Ac+ & \Ac{CAE} & \Ac{MTriplet}\\
		\verb+\acf+ & \acf{CAE} & \acf{MTriplet}\\
		\verb+\Acf+ & \Acf{CAE} & \Acf{MTriplet}\\
		\verb+\acp+   & \acp{CAE} & \acp{MTriplet}\\
		\verb+\Acp+ & \Acp{CAE} & \Acp{MTriplet}\\
		\verb+\acfp+ & \acfp{CAE} & \acfp{MTriplet}\\
		\verb+\Acfp+ & \Acfp{CAE} & \Acfp{MTriplet}\\
		\bottomrule
	\end{tabularx}
	\label{tbl:acro_subsequent_time_examples}
\end{table}

==> background/background.tex <==
\mychapter{Background}{Background}
\label{chap:background}

%Some Chapter introduction.
%
%\input{background/a_section}
%\input{background/summary}

==> background/summary.tex <==
\mysection{Chapter summary}{Chapter Summary}
\label{sec:background_summary}

A summary of what was discussed in this chapter and a small foreshadow of the next Chapter.

==> introduction/contributions_with_related_word.tex <==
\mysubsection{Multimodal speech-vision modelling}{Multimodal Speech-Vision Modelling}
\label{sec:multimodal}

Inspired by the observation that children use co-occurring sensory signals from other modalities to learn a language~\cite{dunbar_interspeech_2021}, some speech models make use of visual grounding as pseudo labels where transcriptions for speech are not available.
Since vision is considered a crucial sensory signal that a child uses during language acquisition~\cite{chrupala_visually_2021}, there has been some interest in speech-vision models~\cite{harwath_jointly_2018, harwath_unsupervised_2016, harwath_learning_2020, harwath_learning_2018, harwath_learning_2017}.
Such models can provide cognitive insights into how children acquire language and provide research into identifying and treating learning disabilities.
Additionally, it can also result in systems for unwritten or low-resource languages: a visual signal could provide a weak form of supervision for speech where it is not possible to obtain transcriptions~\cite{kamper_semantic_2019}.

Recent studies~\cite{sun_look_2016, gupta_visual_2017} have proven that this is a feasible idea by demonstrating that a conventional \ac{ASR} system can be improved by using visual groundings during training.
\citet{kamper_visually_2017} found that this weak supervision provided by the visual groundings enables speech-vision models to capture semantics.
For example, visually grounded speech models are trained to relate an image of a dog either to the word \textit{``dog''} or to the word \textit{``pet''}.
I.e.\ these models learn clusters of semantically relevant concepts like \textit{animal}, \textit{dog} and \textit{pet}.
%With such models, semantics are inferred across various image-caption pairs, as well as within an image-caption pair.
%For example, from the caption \textit{``The brown dog is my pet''}, the model should infer that both \textit{``dog''} and \textit{``pet''} refers to the dog in the image.

Intuitively, for visually grounded models to learn semantic clusters, it should infer that different utterances of the same word belong to the same word class and therefore cluster.
For example, the model should realise that each utterance of the word \textit{``dog''} said by different speakers are of the \textit{dog} word class.
In this way, if anyone says \textit{``dog''}, the model will map this utterance to the cluster \textit{animal--dog--pet}.
I.e.\ to learn semantic clusters, a speech-vision model should learn (1) that different utterances of the same word class have the same acoustics, and (2) that some words are semantically related but differ in acoustics (\textit{``dog''}--\textit{``pet''}) and others are semantically unrelated but have similar acoustics (\textit{``there''}--\textit{``their''}).

Using this complementary relationship between acoustics and semantics to our advantage, we consider speech-vision models to simultaneously learn acoustic and semantic embeddings.
However, we want to explicitly learn separate acoustic and semantic embeddings.  
To our knowledge, \citet{harwath_learning_2020} is the only other study which attempts to separate acoustics and semantics into different embeddings.
Differently than us, they found discrete (categorical) hierarchical acoustic units by using the \myacf{resdavenet} proposed by \citet{harwath_jointly_2018}.
\model{\ac{resdavenet}} is developed through a series of studies.

The first study in this series is \citet{harwath_unsupervised_2016} which proposes the \myacf{davenet} that maps an image and its entire spoken caption to embeddings in a common multimodal space.
Specifically, they use \acp{CNN} to embed an entire audio caption and its matching image into separate fixed-size embeddings. 
The goal is to get embeddings of semantically related images and captions to be more similar than the embeddings of semantically unrelated images and captions.
More specifically, the similarity score $\mathcal{S}$ between semantically related images and captions should be higher than the score for semantically unrelated images and captions.
We follow a similar training procedure between image-caption pairs, but incorporate some of \mycite{harwath_jointly_2018} contributions. 

\begin{figure*}[tb]
	
	\begin{minipage}[htb!]{1.0\textwidth}
		\centering
		\includegraphics[width=0.3\textwidth,height=\textheight,keepaspectratio]{introduction/figures/matchmap_example.png}
	\end{minipage}
	\caption{A matchmap $\mathcal{M}$ localises which regions in an image are semantically related to which regions (a word or multiple words) in the caption, and vice versa. For illustrative purposes we use the learned embedding representing each frame and pixel. A single learned embedding represents a few frames or pixels.}
	\label{fig:matchmap_example}
\end{figure*}

\citet{harwath_jointly_2018} extends the \model{\ac{davenet}} architecture to include residual connections and instead of learning fixed-size embeddings for each caption and image, they learn a sequence of embeddings.
I.e.\ they learn a sequence of embeddings for each image and each caption. %representative of each frame in a spoken caption and each pixel in an image. 
These embedding sequences are then used in a ``matchmap'' $\mathcal{M}$ which aligns the caption embeddings to the image embeddings as illustrated in Figure~\ref{fig:matchmap_example}.
It does so by inferring which word or part of the caption is semantically related to which region(s) in the image, and vice versa.
For the model objective, they calculate a similarity score $\mathcal{S}$ from the matchmap $\mathcal{M}$.

All three of these models~\cite{harwath_unsupervised_2016,harwath_jointly_2018,harwath_learning_2020} use a relative metric to push the similarity score of an image-caption pair $\mathcal{S}_{\im\aud}$ away from the similarity score of a semantically unrelated image-caption pair $\mathcal{S}_{\im'\aud}$ or $\mathcal{S}_{\im\aud'}$. 
Here the apostrophe ($'$) indicates a caption or image that is semantically unrelated to the semantically related image-caption pair $(\im, \aud)$.
%I.e.\ the model explicitly learns which images $I$ and audio captions $A$ are semantically related and which are semantically unrelated. 

In \citet{nortje_direct_2020} and \citet{nortje_direct_2021} we also use a similar relative distance metric to find fixed-size word and image embeddings in a shared multimodal space.
We map a spoken word and image pair to similar embeddings, where an image in a speech-image pair only contains the object corresponding to the paired word. 
%Specifically during training, same concept word and image embeddings are pushed towards one another, while word and image embeddings from different concepts are pushed away from one another.
%This ensures that embeddings of the same concept, regardless of modality, are similar and that embeddings from different concepts are different, regardless of modality.
However, we now aim to embed entire audio captions and images containing multiple objects that may or may not be mentioned in the caption, for four reasons.
The first reason is that natural images consist of more than one object, which leads to our second reason: the entire audio caption relays more semantic information which helps to make sense of the different regions of a natural image. 
Thirdly, if the model can make sense of all the words in a caption and all the objects in an image, then it could also be used in downstream tasks on singular words and objects.
But most importantly, the forth reason is that we believe words before and after a specific word in a sentence relay semantic information about the word. 
This holds for images as well.
For example in the sentence \textit{``The dog catches a ball''} the word \textit{``ball''} relates to the word \textit{``dog''} and \textit{``catches''}.

Some studies have attempted to learn these semantic relationships without the use of visual groundings.
\citet{li_towards_2013}, \citet{harwath_zero_2013} and \citet{chung_speech2vec_2018} attempt to infer semantics between words in a sentence.
\citet{li_towards_2013} and \citet{harwath_zero_2013} use spoken terms which frequently appear together to form semantic relationships between words.
Whereas \citet{chung_speech2vec_2018} finds the \myacf{AWE} of a spoken word and attempts to predict the \model{\acp{AWE}} of the words preceding and succeeding the given word. 
\mydefinition{\aca{AWE}}{is a term used for a single fixed-dimensional representation for a variable duration spoken word segment~\cite{kamper_truly_2019}.}
All three these methods require forced alignments: the actual start and end times of each word in an utterance.
But what if we are working with a zero-resource language and have no access to forced alignments?
To do away with forced alignments and to hopefully learn a metric that can automatically learn word boundaries, we rather use visual groundings in order to build systems for low- or zero-resource languages.


%We setup the multilingual-multimodal setup of \citet{harwath_vision_2018} to train the \myacf{multdavenet} by using \mycite{harwath_unsupervised_2016} \myacf{davenet}.
%Thereafter, we use \model{\ac{multdavenet}} with the matchmap similarity of \citet{harwath_jointly_2018}.
%We are first to use \model{\ac{multdavenet}} with these matchmaps.
%
%Using the \model{\ac{multdavenet}} model, we propose our novel \myacf{accmultdavenet} model consisting of four sub-networks: a visual, an acoustic, an English and a Hindi sub-network.
%As another contribution, we plan to incorporate \ac{CPC} to better capture frame-level acoustic details and the \myacf{resdavenet} of \citet{harwath_learning_2020} to better capture the higher level semantics.
%
%To test the \model{\ac{accmultdavenet}} model, we used the audio and image retrieval tasks of \citet{harwath_unsupervised_2016}.
%We plan to use the visually grounded ZeroSpeech 2021 challenge evaluations of \citet{alishahi_zr-2021vg_2021} to extensively test the model's capabilities.
%Additionally, we will apply the model to a novel downstream word boundary detection task.
%It will be valuable if we can find a method to detect word boundaries in unlabellled speech of zero-resource languages.
%Lastly, we plan to use the \model{\ac{accmultdavenet}} model to mimic \mycite{byers-heinlein_monolingual_2009} cognitive study regarding the disambiguation heuristic.

\mysubsection{Multilingual modelling}{Multilingual Modelling}
\label{sec:multilingual}

\mydefinition{Zero-Resource Languages}{are languages without any transcribed speech resources necessary to develop technology that supports these languages~\cite{jansen_summary_2013, dunbar_zero_2019}.}
\mydefinition{Low-Resource Languages}{are languages with little transcribed speech resources necessary to develop technology that supports these languages.}
To develop systems for low- or zero-resource languages, various studies~\cite{jacobs_acoustic_2021, kamper_multilingual_2020, kamper_improved_2021, hu_multilingual_2020, ma_acoustic_2021} use the idea of multilingual transfer.
\mydefinition{Multilingual Transfer}{is a method that leverages knowledge gained from one or more well-resourced languages to develop systems for low- or zero-resource languages.} 
More specifically, studies in multilingual transfer train a supervised model on labelled data from well-resourced languages and apply the model on an unseen zero-resource language.
For the low-resource setting, they train on the well-resourced languages and update the model on a small labelled dataset from the low-resource language.
We use low-resource and zero-resource interchangeably unless we explicitly refer to the amount of available transcribed speech data.

The idea of multilingual transfer was motivated by the observation that for a specific word class, multilingual infants have to learn the representation of this word in multiple languages~\cite{kovacs_cognitive_2009}.
On top of this, they do so without transcriptions. 
Although this is a very hard task for a machine, we could simultaneously train a speech model to learn the relationship between a well-resourced language and a zero-resource (or a low-resource) language, while providing some supervision in the form of transcriptions on the well-resource side. 
Hopefully, multilingual transfer from the well-resourced side could lead to gains on the zero-resourced side. 

%Since one of our main goals is to develop systems for zero- or low-resource languages, we use multilingual transfer to learn a sequence of acoustic embeddings for a spoken caption.
%However, to our knowledge, the only literature that attempts to use multilingual transfer to learn embeddings for spoken captions, uses joint multilingual and multimodal modelling to learn a fixed-size semantic embedding for the entire caption.
%Hence, we discuss this in Chapter~\ref{sec:jointModelling} where it is more appropriate.
To consider studies that makes use of a pure multilingual setting to learn acoustics, we look into studies that propose \model{\acp{AWE}} or variants thereof in a multilingual training setup. 
%\citet{kamper_improved_2021} and \citet{hermann_multilingual_2021} train \acp{AWE} using multilingual transfer.
\citet{kamper_improved_2021} demonstrates that \model{\acp{AWE}} trained in a multilingual setting outperform \model{\acp{AWE}} trained in an unsupervised setting on unlabelled data.
Following the findings of \citet{kamper_improved_2021}, \citet{jacobs_acoustic_2021} asks whether unsupervised learning and multilingual transfer could be complementary; they pretrain an \model{\ac{AWE}} model on labelled data from well-resourced languages before training on unlabelled data from a zero-resource language. 
They demonstrate that this combined method outperforms the purely unsupervised or multilingual transfer methods.
We also train our models on audio without transcriptions by using multilingual transfer between the well-resourced language and the zero-resource language.

%Similarly as \citet{ma_acoustic_2021}, we will train on two languages: a well resourced language and a zero-resource language. 
%\citet{ma_acoustic_2021} specifically trained multilingual \acp{AWE} on these two languages and used it in a \ac{QbE} task. \lntodo{They call it BNF and not AWE.But accoring toe the AWE definition above,  I see it as the same thing in this setup. Is that wrong?}
%\Ac{QbE} is the task of finding utterances in which a keyword (the query) occurs by using its audio frames. This is a specialised instance of the \ac{STD} method~\cite{ma_acoustic_2021, hu_acoustic_2021}.

\citet{hu_multilingual_2020} uses multiple well-resourced languages to train a multilingual model consisting of an \model{\ac{AWE}} and an \myacf{AGWE} model.
\mydefinition{\aca{AGWE}}{is an embedding which represents a word's phonetic content~\cite{hu_multilingual_2020}.}
Although the \model{\ac{AGWE}} side requires phonetically transcribed data, the \model{\ac{AGWE}} branch is used during training to improve the \model{\ac{AWE}} model.
After training, the \model{\ac{AWE}} model can be used on its own to embed words from an unseen zero-resource language.  
We do not incorporate this method in out basic setup, but this could be adapted for our setting to improve the acoustics of the well-resourced language, which in turn could improve the acoustics of the zero-resource language and the learned semantics. 

Our main goal is to learn separate acoustic and semantic embeddings.
Therefore, we train on entire caption utterances since we argue that an entire utterance relays more semantics than considering each word in the utterance in isolation. 
This is similar to \citet{hu_acoustic_2021} which proposes an \myacf{ASE} model trained on entire utterances.
An \model{\ac{ASE}} model uses the idea of an \model{\ac{AWE}} model, but instead of a single word it takes in spans of words and outputs a single embedding for multiple words. 
However, we learn embedding sequences for each caption since we use matchmaps to align each caption frame and pixel.

Although \citet{hermann_multilingual_2021} shows that using multiple well-resourced languages leads to acoustic embedding sequences that better capture the acoustics across languages, we are limited in the amount of well-resourced languages that can be paired up with images and captions from a zero-resource language.
Similarly as \citet{ma_acoustic_2021}, we will train on two languages: a well resourced language and a zero-resource language.

\mysubsection{Multilingual speech-vision modelling}{Multilingual Speech-Vision Modelling}
\label{sec:jointModelling}

\Acf{ASR} is facing two major hurdles. 
The first is obtaining systems for zero-resource languages where transcriptions cannot be collected~\cite{dunbar_interspeech_2021, dunbar_zero_2020, dunbar_zero_2019}.
To address this, research focussed on using co-occurring visual signals as pseudo-labels for speech as discussed in Chapter~\ref{sec:multimodal}.
The second hurdle is the dependency of current \ac{ASR} systems on large amounts of transcribed data~\cite{kamper_unsupervised_2017}.
As a solution to this hurdle, recent research uses the idea that knowledge gained from large datasets of well-resourced languages can be utilised to produce acoustic embeddings for zero-resource languages as discussed in Chapter~\ref{sec:multilingual}.
We combine these two solutions into a multilingual-multimodal model which learns semantic mappings between two captions from different languages and the image associated with these two captions.  

There are only a hand full of similar studies that model captions from different languages and co-occurring images to a shared embedding space. 
The first noteworthy study by \citet{harwath_vision_2018} mapped associated Hindi captions, English captions and images to a joint space. 
The model uses the \model{\ac{davenet}}~\cite{harwath_unsupervised_2016} architecture discussed in Chapter~\ref{sec:multimodal}, but adds another audio branch to the architecture.
The entire Chapter~\ref{chap:baseStudy} is dedicated to discussing and reproducing this study since we base our model on theirs.

\citet{harwath_vision_2018} uses a multilingual-multimodal triplet-like loss to push semantically related images and captions towards each other while pushing semantically unrelated images and captions away from one another.
\citet{ohishi_pair_2020} uses the same model as \citet{harwath_vision_2018} on Japanese and English data.
Moreover, they use a pair expansion scheme that requires two datasets consisting of images and spoken captions.
The datasets should be from different languages and their image sets should be disjoint. 
The captions in these two datasets are then paired up according to image similarity between the sets. 
In this way, two captions from different languages can be mapped to each other, as well as each caption to their own image.
%This dataset pair expansion scheme could be valuable for us to pair an audio-image dataset from a well-resourced language and an audio-image dataset from a zero-resource langauge for ablation experiments.

%\citet{azuh_towards_2019} also uses \mycite{harwath_vision_2018} model to segment the spoken captions within each language into regions which approximately correspond to words. 
%These regions are then mean-pooled and clustered according to pseudo-words for each language.
%English pseudo-clusters are associated to Hindi pseudo-word clusters according to dot product similarities between cluster centroids.
%\citet{azuh_towards_2019} shows that semantic translations between English and Hindi words are captured by many of these paired up clusters.
%This is a valuable downstream task we want to test our models on: can we translate captions from a zero-resource language to a well-resourced language like English?
%This could be helpful to adapt well developed systems to support zero-resource languages.

Another study by \citet{kamper_visually_2018} constructs their own multilingual-multimodal dataset by using a German visual tagger to describe the image in an English image-caption pair with German text.
Their model which found valuable semantic translations, consists of two sub-networks: one network is the German visual tagger which maps an image to a German description while the other network maps the training image's spoken English caption to the generated German text. 
This system is developed for cross-lingual keyword spotting: given a text keyword in a language with a written form, we can find all the spoken utterances containing that keyword in another zero-resource language.   
Although English is used as the zero-resource language, this study is only a proof-of-concept that multilingual transfer together with visual grounding could be used to build systems for zero-resource languages. 

%Although text from the well-resourced side may be useful, we will start with the matchmap model of \citet{harwath_vision_2018} since it could be useful to a wider variety of tasks and later be altered to incorporate text.

==> multilingual_mutual_exclusivity/background.tex <==
\mysection{Related work}{Related Work}

\subsection{Multilingual ME}

\subsubsection{Monolingual, bilingual, trilingual: infants' language experience influences the development of a word-learning heuristic -- Byers-Heinlein and Werker~\cite{byers-heinlein_monolingual_2009}}

\textbf{What?}
They investigate where the ME bias used by 17- to 18-month-old infants originate from.
More specifically, they investigate the influence of an infant's language background on the ME bias they show. 

\textbf{How?} 
They used three familiar classes: ``car'', ``ball'' and ``shoe''. 
And one novel class where the image class was that of a phototube and the word class was ``nil''. 
They tested the children on two of the familiar classes, and then on the novel class using the remaining familiar class. 

\textbf{Conclusion?}
Monolingual infants showed a strong use of ME.
Bilingual infants showed marginal use of the bias, whereas trilingual infants showed no usage of the bias. 
I.e. the number of languages being learned by the infant, predicted ME performance. 

\textbf{Useful stuff}
\begin{enumerate}
	\item Translation equivalents represent a departure from the one-to-one mapping between word and concept that is  typical of  monolingual  vocabularies. Trilinguals might know even more translation equivalents than bilinguals. Language experience could influence early disambiguation  because  knowledge of  many-to-one mappings delays its development in the multilingual, because knowledge of one-to-one mappings promotes its development in the monolingual, or through an interplay of both factors.
\end{enumerate}


 \subsubsection{Bilingualism in the early years: What the science says -- Byers-Heinlein and Lew-Williams~\cite{byers-heinlein_bilingualism_2013}}

 \textbf{What?}

 \textbf{How?}

 \textbf{Conclusion?}
 
 
 \subsubsection{\cite{kalashnikova_effects_2015}}

==> visually_grounded_few-shot_word_acquisition/background_raw.tex <==


